Continuous vs. Discrete Optimization of Deep Neural Networks

Existing analyses of optimization in deep learning are either continuous, focusing on (variants of) gradient flow, or discrete, directly treating (variants of) gradient descent. Gradient flow is amenable to theoretical analysis, but is stylized and disregards computational efficiency. The extent to which it represents gradient descent is an open question in the theory of deep learning. The current paper studies this question. Viewing gradient descent as an approximate numerical solution to the initial value problem of gradient flow, we find that the degree of approximation depends on the curvature around the gradient flow trajectory. We then show that over deep neural networks with homogeneous activations, gradient flow trajectories enjoy favorable curvature, suggesting they are well approximated by gradient descent. This finding allows us to translate an analysis of gradient flow over deep linear neural networks into a guarantee that gradient descent efficiently converges to global minimum almost surely under random initialization. Experiments suggest that over simple deep neural networks, gradient descent with conventional step size is indeed close to gradient flow. We hypothesize that the theory of gradient flows will unravel mysteries behind deep learning.

==> sec_outline.tex <==
%\section{Introduction}
%
%Significant efforts are being invested in studying gradient-based optimization of deep neural networks (in terms of both convergence and implicit regularization).
%There is a dichotomy between continuous and discrete analyses.
%The former allow use of powerful mathematical machinery, and typically give rise to stronger results.
%The latter on the other hand represents the algorithms that run in practice, taking into account the critical aspect of computational efficiency.
%To date, little is known about the relationship between continuous and discrete optimization of deep neural networks.
%The current paper addresses this question.
%Viewing gradient descent as a discrete approximation of the solution to the gradient flow ODE, we turn to the literature on numerical integration, and invoke a powerful theorem by Dahlquist.
%The theorem implies that the match between gradient flow and gradient descent is determined by convexity.
%More specifically, the larger the most negative eigenvalue of the Hessian is, the larger the learning rate of gradient descent can be.
%Despite the fact that over arbitrary non-convex objectives the learning rate must be exponentially small, we show that over fully-connected deep neural networks with homogeneous (linear or ReLU) activation, gradient flow traverses through path that is ``roughly convex'', in the sense that the magnitude of the most negative Hessian eigenvalue along this path is much smaller than in other points in space.
%This suggests that for deep neural networks, gradient descent with reasonably small learning rate is in fact close to the continuous limit (\ie~to gradient flow).
%We make use of the result and conduct a refined analyses for the linear activation case, deriving the first global convergence result for arbitrarily deep neural networks.
%Our analysis is corroborated by experiments, in the setting we analyze as well as more realistic deep learning settings.
%
%The main contributions of the paper are:
%\begin{itemize}
%\item We conduct the first formal study of the discrepancy between continuous and discrete optimization of deep neural networks.
%\item We provide what is, to the best of our knowledge, the first demonstration of how generic machinery can be used to translate a continuous non-convex convergence result into a discrete one.
%\item The discrete result we derive forms the first guarantee of convergence to global minimum for deep (three or more layer) neural networks taking place almost surely with respect to data-independent initialization.
%\item The mathematical tools we employ are not well known in the machine learning community and may be of independent interest.
%\end{itemize}

%\section{Related work}
%
%Should cover: continuous and discrete analyses of optimization in deep learning, papers connecting the two (by Bach, Rene Vidal and more), related works outside of deep learning.
%
%Relevant works:
%\begin{itemize}
%\item \href{https://arxiv.org/abs/1806.00900}{Algorithmic Regularization in Learning Deep Homogeneous Models: Layers are Automatically Balanced}
%\item \href{https://arxiv.org/abs/1702.06751}{Integration Methods and Accelerated Optimization Algorithms}
%\item \href{https://arxiv.org/abs/1805.00521}{Direct Runge-Kutta Discretization Achieves Acceleration}
%\item \href{https://arxiv.org/abs/2012.04728}{Neural Mechanics: Symmetry and Broken Conservation Laws in Deep Learning Dynamics}
%\item \href{https://arxiv.org/abs/2009.11162}{Implicit Gradient Regularization}
%\item \href{https://arxiv.org/abs/1503.01243}{A Differential Equation for Modeling Nesterov's Accelerated Gradient Method: Theory and Insights}
%\item Papers by \href{https://scholar.google.com/citations?hl=en&user=svlR9_cAAAAJ&view_op=list_works&sortby=pubdate}{Guilherme Starvaggi Franca} and references therein
%\item \href{https://arxiv.org/abs/2004.08981}{Stochastic gradient algorithms from ODE splitting perspective}
%\item \href{https://arxiv.org/abs/1811.01558}{Stochastic Modified Equations and Dynamics of Stochastic Gradient Algorithms I: Mathematical Foundations} and other papers by \href{https://scholar.google.com/citations?user=i2mOt14AAAAJ&hl=en&oi=ao}{Weinan E}
%\item Analyses of convergence to global minimum for gradient-based algorithms over deep models (make sure convergence doesn't take place almost surely!) 
%\end{itemize}

%\section{Preliminaries}
%
%Euler's method for approximating initial value problems, Dahlquist's theorem

%\section{Continuous vs.~Discrete Optimization: Match Determined by Convexity}
%
%Specialize Dahlquist's theorem to gradient flow \vs~gradient descent for each of the following cases:
%\emph{(i)}~strongly convex objective;
%\emph{(ii)}~(non-strongly) convex objective;
%and
%\emph{(iii)}~non-convex objective.
%For each case, provide an example showing that Dahlquist's theorem is tight (\ie~there exist objectives on which the error evolves as in Dahlquist's theorem).
%The message of this section is that the determining factor in terms of the match between gradient flow and gradient descent is convexity.
%It may seem like having a match in the non-convex case is hopeless, but actually, if the objective is ``roughly convex'' around the gradient flow path then it is possible.

%\section{Optimization of Deep Neural Networks is Roughly Convex}
%
%Present model of fully-connected/convolutional deep neural network with homogeneous activation (linear or ReLU) performing scalar regression (single output, $\ell_2$~loss).
%Using known conservation laws (Du~\etal~paper) prove that the most negative Hessian around gradient flow path is ``not too negative'', and gets less and less negative as the global optimum is approached.
%The message here is that although deep neural networks admit non-convex training objectives, they are ``roughly convex'' around gradient flow paths, and hence do give rise to a match between gradient flow and gradient descent.

%\section{A Refined Analysis for Deep Linear Neural Networks}
%
%In this section we show how the findings of the previous section can be used to derive a new global convergence result for gradient descent.
%We will first lay out a proposition for gradient flow (starting from balanced initialization), and then as a corollary of that and Dahlquist's theorem we will obtain a theorem for gradient descent.
%A corollary of this theorem will be that under balanced initialization convergence can be guaranteed with probability close to 1.
%We will mention that not only do we know that gradient descent converges, but we also know which path it takes (perhaps including an illustrating figure).

%\section{Experiments}
%
%Two types of experiments can be presented:
%\emph{(i)}~comparison of gradient descent paths under different learning rates;
%and
%\emph{(ii)}~evaluation of Hessian spectrum on gradient descent path and away from it.
%The analyzed model can be evaluated with both linear and ReLU activation, and we can also evaluate more realistic models (\eg~LeNet on MNIST).

%\section{Conclusion}
%
%Summarize and provide outlook towards the future.
%Some possibilities for the latter: encouragement to continue analyzing continuous optimization algorithms; something about rough convexity around optimization trajectories (perhaps raise potential practical implications).

